The Stereotyping Problem in Collaboratively Filtered Recommender Systems

Recommender systems play a crucial role in mediating our access to online information. We show that such algorithms induce a particular kind of stereotyping: if preferences for a set of items are anti-correlated in the general user population, then those items may not be recommended together to a user, regardless of that user's preferences and rating history. First, we introduce a notion of joint accessibility, which measures the extent to which a set of items can jointly be accessed by users. We then study joint accessibility under the standard factorization-based collaborative filtering framework, and provide theoretical necessary and sufficient conditions when joint accessibility is violated. Moreover, we show that these conditions can easily be violated when the users are represented by a single feature vector. To improve joint accessibility, we further propose an alternative modelling fix, which is designed to capture the diverse multiple interests of each user using a multi-vector representation. We conduct extensive experiments on real and simulated datasets, demonstrating the stereotyping problem with standard single-vector matrix factorization models.

==> facctrec_style.tex <==
% packages
\usepackage{diagbox}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{tikz,tikz-3dplot}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{url,ifthen}
\usepackage{enumitem}
\usepackage{srcltx}
\usepackage{multirow}
\usepackage{boxedminipage}
% \usepackage[margin=1.1in]{geometry}
\usepackage{nicefrac}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{color}
\usepackage{subfig}
\usepackage{colortbl}
\usepackage{setspace}
\usepackage{pgfplots}
\pgfplotsset{compat=1.12}
\usepackage{algorithm,algorithmic}
% \usepackage[algo2e]{algorithm2e}

\usepackage{xcolor}
\definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
\definecolor{DarkRed}{rgb}{0.5,0.1,0.1}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{Gray}{rgb}{0.2,0.2,0.2}

\definecolor{c1}{RGB}{38, 70, 83}
\definecolor{c2}{RGB}{42, 157, 143}
\definecolor{c3}{RGB}{233, 196, 106}
\definecolor{c5}{RGB}{231, 111, 81}
\definecolor{c4}{RGB}{244, 162, 97}



\definecolor{c1}{RGB}{38, 70, 83}
\definecolor{c2}{RGB}{42, 157, 143}
\definecolor{c3}{RGB}{233, 196, 106}
\definecolor{c5}{RGB}{231, 111, 81}
\definecolor{c4}{RGB}{244, 162, 97}
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\renewcommand{\ttdefault}{pcr}
\usepackage{listings}
\lstdefinestyle{mystyle}{
    commentstyle=\color{DarkBlue},
    keywordstyle=\color{DarkRed},
    numberstyle=\tiny\color{Gray},
    stringstyle=\color{DarkGreen},
    basicstyle=\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}


% \usepackage[small]{caption}
\usepackage{caption}
% \usepackage{hyperref}


% 1 for working draft
% will show author notes
\def\draft{0}

% 1 for submission version
% set to zero after submission
% use \forsubmit{visible during submission}
% and \forreals{visible after submission}
\def\submit{0}

\ifnum\draft=1 % show authors' note if draft
    \def\ShowAuthNotes{1}
\else
    \def\ShowAuthNotes{0}
\fi

\ifnum\submit=1
\newcommand{\forsubmit}[1]{#1}
\newcommand{\forreals}[1]{}
\else
\newcommand{\forreals}[1]{#1}
\newcommand{\forsubmit}[1]{}
\fi

% theorem environments

\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}[theorem]{Remark}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}%[section]
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openQ}[theorem]{Open Question}


% % option to continue an example
% \newtheoremstyle{example_contd}
% {\topsep} {\topsep}%
% {}% Body font
% {}% Indent amount (empty = no indent, \parindent = para indent)
% {\bfseries}% Thm head font
% {.}% Punctuation after thm head
% {1em}% Space after thm head (\newline = linebreak)
% {\thmname{#1} \thmnumber{ #2}\thmnote{#3} (continued)}% Thm head spec

% \theoremstyle{example_contd}
% \newtheorem*{example_contd}{Example}

%
% nice refs
%
\newcommand{\chapterlabel}[1]{\label{ch:#1}}
\newcommand{\chapterref}[1]{Chapter~\ref{ch:#1}}
\newcommand{\claimlabel}[1]{\label{claim:#1}}
\newcommand{\claimref}[1]{Claim~\ref{claim:#1}}
\newcommand{\corollarylabel}[1]{\label{cor:#1}}
\newcommand{\corollaryref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\definitionlabel}[1]{\label{def:#1}}
\newcommand{\definitionref}[1]{Definition~\ref{def:#1}}
\newcommand{\equationlabel}[1]{\label{eq:#1}}
\newcommand{\equationref}[1]{Equation~\ref{eq:#1}}
\newcommand{\factlabel}[1]{\label{fact:#1}}
\newcommand{\factref}[1]{\Fact~\ref{fact:#1}}
\newcommand{\figurelabel}[1]{\label{fig:#1}}
\newcommand{\figureref}[1]{\Figure~\ref{fig:#1}}
\newcommand{\tablelabel}[1]{\label{tab:#1}}
\newcommand{\tableref}[1]{Table~\ref{tab:#1}}
\newcommand{\itemlabel}[1]{\label{item:#1}}
\newcommand{\itemref}[1]{Item~(\ref{item:#1})}
\newcommand{\lemmalabel}[1]{\label{lem:#1}}
\newcommand{\lemmaref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\propositionlabel}[1]{\label{prop:#1}}
\newcommand{\propositionref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\remarklabel}[1]{\label{rem:#1}}
\newcommand{\remarkref}[1]{Remark~\ref{rem:#1}}
\newcommand{\sectionlabel}[1]{\label{sec:#1}}
\newcommand{\sectionref}[1]{\Section~\ref{sec:#1}}
\newcommand{\theoremlabel}[1]{\label{thm:#1}}
\newcommand{\theoremref}[1]{Theorem~\ref{thm:#1}}


%
% nice fonts
%
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{kpfonts}
% \usepackage{microtype}

% Expectation, Probability, Variance
\newcommand{\E}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}
% \DeclareMathOperator*{\E}{\Esymb}
% \DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb r}
\renewcommand{\Pr}{\ProbOp}
% \newcommand{\Prob}{\mathbb{P}}
% \newcommand{\prob}[1]{\Pr\big\{ #1 \big\}}
% \newcommand{\Prob}[1]{\Pr\left\{ #1 \right\}}
\newcommand{\varprob}[1]{\Pr\big( #1 \big)}
\newcommand{\varProb}[1]{\Pr\left( #1 \right)}
\newcommand{\ex}[1]{\E\big[#1\big]}
\newcommand{\Ex}[1]{\E\left[#1\right]}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}
% \newcommand{\widebar}[1]{\overline{#1}}
\newcommand{\tv}{\text{TV}}

% nice fractions
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\nfrac}{\nicefrac}
\newcommand{\half}{\nfrac12}
\newcommand{\quarter}{\nfrac14}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

\renewcommand{\hat}{\widehat}

% cally fonts
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

% binary relations
\newcommand{\defeq}{\stackrel{\small \mathrm{def}}{=}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}
% parentheses
% \newcommand{\paren}[1]{(#1 )}
\newcommand{\Paren}[1]{\left(#1 \right )}
% brackets
\newcommand{\brac}[1]{[#1 ]}
\newcommand{\Brac}[1]{\left[#1 \right]}
% set braces
\newcommand{\set}[1]{\{#1\}}
\newcommand{\bigset}[1]{\bigl\{#1\bigr\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
% absolute value sign
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\Bigabs}[1]{\Bigl\lvert#1\Bigr\rvert}
% \newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert_2}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
% declare function f as $f \from X \to Y$
\newcommand{\from}{\colon}
% differential as in "\int x\rd x"
\newcommand\rd{\,\mathrm{d}}
% sets
\newcommand{\bits}{\{0,1\}}
\newcommand{\signs}{\{-1,1\}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb Z}
\newcommand{\D}{\mathcal D}
% \newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\varR}{\Re}
\newcommand{\Rnn}{\R_+}
\newcommand{\varRnn}{\varR_+}
% qed symbol
\renewcommand{\qedsymbol}{{$\blacksquare$}}
% bold vector notation
\usepackage{bm}
\renewcommand{\vec}[1]{{\bm{#1}}}

% linear algebra
% \DeclareMathOperator*{\range}{range}
\newcommand{\Mid}{\ensuremath{~\Big|~}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\trans}{\top}
\newcommand{\pinv}{\dagger}
\newcommand{\iprod}[1]{\langle #1\rangle}
\newcommand{\isqur}[1]{\langle #1,#1\rangle}
\newcommand{\trsp}[1]{#1^\dagger}
\newcommand{\vartrsp}[1]{#1^T}
\newcommand{\varvartsp}[1]{#1^{\mathsf{T}}}
\newcommand{\smallrmtrsp}[1]{#1^{\scriptscriptstyle \mathrm{T}}}
\newcommand{\oprod}[2]{\trsp{#1} #2}
\newcommand{\osqur}[1]{\oprod{#1}{#1}}
% transposed of a vector
\newcommand{\trspvec}[1]{{\trsp{\vec{#1}}}}
% norm
\newcommand{\snorm}[1]{\norm{#1}^2}
% L2 norm
\newcommand{\normt}[1]{\norm{#1}_{\scriptstyle 2}}
\newcommand{\varnormt}[1]{\norm{#1}_{\scriptscriptstyle 2}}
\newcommand{\snormt}[1]{\normt{#1}^2}
% L1 norm
\newcommand{\normo}[1]{\norm{#1}_{\scriptstyle 1}}
\newcommand{\Normo}[1]{\Norm{#1}_{\scriptstyle 1}}
\newcommand{\varnormo}[1]{\norm{#1}_{\scriptscriptstyle 1}}
% Linfty norm
\newcommand{\normi}[1]{\norm{#1}_{\scriptstyle \infty}}
\newcommand{\varnormi}[1]{\norm{#1}_{\scriptscriptstyle \infty}}

% super set with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% Indictator function
\newcommand{\Ind}{\mathbb I}

% common abbrevs
\newcommand{\ignore}[1]{}
\newcommand{\OPT}{\mathrm{OPT}}
\newcommand{\opt}{\mathrm{opt}}
% \newcommand{\KL}{\mathrm{KL}}
\newcommand{\sign}{\mathit{sign}}
\newcommand{\polylog}{{\rm polylog}}
\newcommand{\poly}{{\rm poly}}
% \newcommand{\vol}{\mathrm{vol}}
\newcommand{\supp}{\mathrm{supp}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\reg}{\text{reg}}

% epsilon wars
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}

% distributions
\newcommand{\Laplace}{\mathrm{Lap}}
\newcommand{\Lap}{\Laplace}
\newcommand{\Bin}{\mathrm{Bin}}


% remove text
\newcommand{\remove}[1]{}

%
% draftbox
%
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
        \begin{Large}%
          \textsc{Working Draft}%
        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}

% compact itemize and enumerate
\renewcommand{\labelitemi}{--}
\newenvironment{itm}
{\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]}
{\end{itemize}}
\newenvironment{enum}
{\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]}
{\end{enumerate}}

% control white space of list and display environments
%
%\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
%\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}
\def\mydatewithyear{\leavevmode\hbox{\the\year/\twodigits\month/\twodigits\day}}
\def\twodigits#1{\ifnum#1<10 0\fi\the#1}
\def\mydate{\leavevmode\hbox{\twodigits\month/\twodigits\day}}
\def\twodigits#1{\ifnum#1<10 0\fi\the#1}

% Macros for repeated theorems.
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newreptheorem{theorem}{Theorem}
\newreptheorem{corollary}{Corollary}
\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}




\newcounter{protocol}
\makeatletter
\newenvironment{protocol}[1][htb]{%
  \let\c@algorithm\c@protocol
  \renewcommand{\ALG@name}{Procedure}% Update algorithm name
  \begin{algorithm}[#1]%
  }{\end{algorithm}
}
\makeatother


==> wg_style.tex <==
% packages
\usepackage{diagbox}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{tikz,tikz-3dplot}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{url,ifthen}
\usepackage[square,sort,comma,numbers]{natbib}
\usepackage{enumitem}
\usepackage{srcltx}
\usepackage{multirow}
\usepackage{boxedminipage}
% \usepackage[margin=1.1in]{geometry}
\usepackage{nicefrac}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{color}
\usepackage{subfig}
\usepackage{colortbl}
\usepackage{setspace}
\usepackage{pgfplots}
\pgfplotsset{compat=1.12}
\usepackage{algorithm,algorithmic}
% \usepackage[algo2e]{algorithm2e}

\usepackage{xcolor}
\definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
\definecolor{DarkRed}{rgb}{0.5,0.1,0.1}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{Gray}{rgb}{0.2,0.2,0.2}

\definecolor{c1}{RGB}{38, 70, 83}
\definecolor{c2}{RGB}{42, 157, 143}
\definecolor{c3}{RGB}{233, 196, 106}
\definecolor{c5}{RGB}{231, 111, 81}
\definecolor{c4}{RGB}{244, 162, 97}



\definecolor{c1}{RGB}{38, 70, 83}
\definecolor{c2}{RGB}{42, 157, 143}
\definecolor{c3}{RGB}{233, 196, 106}
\definecolor{c5}{RGB}{231, 111, 81}
\definecolor{c4}{RGB}{244, 162, 97}
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\renewcommand{\ttdefault}{pcr}
\usepackage{listings}
\lstdefinestyle{mystyle}{
    commentstyle=\color{DarkBlue},
    keywordstyle=\color{DarkRed},
    numberstyle=\tiny\color{Gray},
    stringstyle=\color{DarkGreen},
    basicstyle=\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}


% \usepackage[small]{caption}
\usepackage{caption}
\usepackage{hyperref}
\hypersetup{
    unicode=false,          % non-Latin characters in AcrobatÂ¿s bookmarks
    pdftoolbar=true,        % show Acrobat toolbar?
    pdfmenubar=true,        % show Acrobat menu?
    pdffitwindow=false,      % page fit to window when opened
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=DarkBlue,          % color of internal links
    citecolor=DarkGreen,        % color of links to bibliography
    filecolor=DarkRed,      % color of file links
    urlcolor=DarkBlue,          % color of external links
    %
    % paper specific, please update
    %
    pdftitle={},
    pdfauthor={},
}


% 1 for working draft
% will show author notes
\def\draft{1}

% 1 for submission version
% set to zero after submission
% use \forsubmit{visible during submission}
% and \forreals{visible after submission}
\def\submit{0}

\ifnum\draft=1 % show authors' note if draft
    \def\ShowAuthNotes{1}
\else
    \def\ShowAuthNotes{0}
\fi

\ifnum\submit=1
\newcommand{\forsubmit}[1]{#1}
\newcommand{\forreals}[1]{}
\else
\newcommand{\forreals}[1]{#1}
\newcommand{\forsubmit}[1]{}
\fi

% theorem environments

\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}[theorem]{Remark}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}%[section]
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openQ}[theorem]{Open Question}


% % option to continue an example
% \newtheoremstyle{example_contd}
% {\topsep} {\topsep}%
% {}% Body font
% {}% Indent amount (empty = no indent, \parindent = para indent)
% {\bfseries}% Thm head font
% {.}% Punctuation after thm head
% {1em}% Space after thm head (\newline = linebreak)
% {\thmname{#1} \thmnumber{ #2}\thmnote{#3} (continued)}% Thm head spec

% \theoremstyle{example_contd}
% \newtheorem*{example_contd}{Example}

%
% nice refs
%
\newcommand{\chapterlabel}[1]{\label{ch:#1}}
\newcommand{\chapterref}[1]{\hyperref[ch:#1]{Chapter~\ref{ch:#1}}}
\newcommand{\claimlabel}[1]{\label{claim:#1}}
\newcommand{\claimref}[1]{\hyperref[claim:#1]{Claim~\ref{claim:#1}}}
\newcommand{\corollarylabel}[1]{\label{cor:#1}}
\newcommand{\corollaryref}[1]{\hyperref[cor:#1]{Corollary~\ref{cor:#1}}}
\newcommand{\definitionlabel}[1]{\label{def:#1}}
\newcommand{\definitionref}[1]{\hyperref[def:#1]{Definition~\ref{def:#1}}}
\newcommand{\equationlabel}[1]{\label{eq:#1}}
\newcommand{\equationref}[1]{\hyperref[eq:#1]{Equation~\ref{eq:#1}}}
\newcommand{\factlabel}[1]{\label{fact:#1}}
\newcommand{\factref}[1]{\hyperref[fact:#1]{Fact~\ref{fact:#1}}}
\newcommand{\figurelabel}[1]{\label{fig:#1}}
\newcommand{\figureref}[1]{\hyperref[fig:#1]{Figure~\ref{fig:#1}}}
\newcommand{\tablelabel}[1]{\label{tab:#1}}
\newcommand{\tableref}[1]{\hyperref[tab:#1]{Table~\ref{tab:#1}}}
\newcommand{\itemlabel}[1]{\label{item:#1}}
\newcommand{\itemref}[1]{\hyperref[item:#1]{Item~(\ref{item:#1})}}
\newcommand{\lemmalabel}[1]{\label{lem:#1}}
\newcommand{\lemmaref}[1]{\hyperref[lem:#1]{Lemma~\ref{lem:#1}}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{\hyperref[prop:#1]{Proposition~\ref{prop:#1}}}
\newcommand{\propositionlabel}[1]{\label{prop:#1}}
\newcommand{\propositionref}[1]{\hyperref[prop:#1]{Proposition~\ref{prop:#1}}}
\newcommand{\remarklabel}[1]{\label{rem:#1}}
\newcommand{\remarkref}[1]{\hyperref[rem:#1]{Remark~\ref{rem:#1}}}
\newcommand{\sectionlabel}[1]{\label{sec:#1}}
\newcommand{\sectionref}[1]{\hyperref[sec:#1]{Section~\ref{sec:#1}}}
\newcommand{\theoremlabel}[1]{\label{thm:#1}}
\newcommand{\theoremref}[1]{\hyperref[thm:#1]{Theorem~\ref{thm:#1}}}


%
% nice fonts
%
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{kpfonts}
% \usepackage{microtype}

% Expectation, Probability, Variance
\newcommand{\E}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}
% \DeclareMathOperator*{\E}{\Esymb}
% \DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb r}
\renewcommand{\Pr}{\ProbOp}
% \newcommand{\Prob}{\mathbb{P}}
% \newcommand{\prob}[1]{\Pr\big\{ #1 \big\}}
% \newcommand{\Prob}[1]{\Pr\left\{ #1 \right\}}
\newcommand{\varprob}[1]{\Pr\big( #1 \big)}
\newcommand{\varProb}[1]{\Pr\left( #1 \right)}
\newcommand{\ex}[1]{\E\big[#1\big]}
\newcommand{\Ex}[1]{\E\left[#1\right]}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}
% \newcommand{\widebar}[1]{\overline{#1}}
\newcommand{\tv}{\text{TV}}

% nice fractions
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\nfrac}{\nicefrac}
\newcommand{\half}{\nfrac12}
\newcommand{\quarter}{\nfrac14}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

\renewcommand{\hat}{\widehat}

% cally fonts
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% binary relations
\newcommand{\defeq}{\stackrel{\small \mathrm{def}}{=}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}
% parentheses
% \newcommand{\paren}[1]{(#1 )}
\newcommand{\Paren}[1]{\left(#1 \right )}
% brackets
\newcommand{\brac}[1]{[#1 ]}
\newcommand{\Brac}[1]{\left[#1 \right]}
% set braces
\newcommand{\set}[1]{\{#1\}}
\newcommand{\bigset}[1]{\bigl\{#1\bigr\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
% absolute value sign
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\Bigabs}[1]{\Bigl\lvert#1\Bigr\rvert}
% \newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert_2}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
% declare function f as $f \from X \to Y$
\newcommand{\from}{\colon}
% differential as in "\int x\rd x"
\newcommand\rd{\,\mathrm{d}}
% sets
\newcommand{\bits}{\{0,1\}}
\newcommand{\signs}{\{-1,1\}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb Z}
\newcommand{\D}{\mathcal D}
\newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\varR}{\Re}
\newcommand{\Rnn}{\R_+}
\newcommand{\varRnn}{\varR_+}
% qed symbol
\renewcommand{\qedsymbol}{{$\blacksquare$}}
% bold vector notation
\usepackage{bm}
\renewcommand{\vec}[1]{{\bm{#1}}}

% linear algebra
% \DeclareMathOperator*{\range}{range}
\newcommand{\Mid}{\ensuremath{~\Big|~}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\trans}{\top}
\newcommand{\pinv}{\dagger}
\newcommand{\iprod}[1]{\langle #1\rangle}
\newcommand{\isqur}[1]{\langle #1,#1\rangle}
\newcommand{\trsp}[1]{#1^\dagger}
\newcommand{\vartrsp}[1]{#1^T}
\newcommand{\varvartsp}[1]{#1^{\mathsf{T}}}
\newcommand{\smallrmtrsp}[1]{#1^{\scriptscriptstyle \mathrm{T}}}
\newcommand{\oprod}[2]{\trsp{#1} #2}
\newcommand{\osqur}[1]{\oprod{#1}{#1}}
% transposed of a vector
\newcommand{\trspvec}[1]{{\trsp{\vec{#1}}}}
% norm
\newcommand{\snorm}[1]{\norm{#1}^2}
% L2 norm
\newcommand{\normt}[1]{\norm{#1}_{\scriptstyle 2}}
\newcommand{\varnormt}[1]{\norm{#1}_{\scriptscriptstyle 2}}
\newcommand{\snormt}[1]{\normt{#1}^2}
% L1 norm
\newcommand{\normo}[1]{\norm{#1}_{\scriptstyle 1}}
\newcommand{\Normo}[1]{\Norm{#1}_{\scriptstyle 1}}
\newcommand{\varnormo}[1]{\norm{#1}_{\scriptscriptstyle 1}}
% Linfty norm
\newcommand{\normi}[1]{\norm{#1}_{\scriptstyle \infty}}
\newcommand{\varnormi}[1]{\norm{#1}_{\scriptscriptstyle \infty}}

% super set with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% Indictator function
\newcommand{\Ind}{\mathbb I}

% common abbrevs
\newcommand{\ignore}[1]{}
\newcommand{\OPT}{\mathrm{OPT}}
\newcommand{\opt}{\mathrm{opt}}
% \newcommand{\KL}{\mathrm{KL}}
\newcommand{\sign}{\mathit{sign}}
\newcommand{\polylog}{{\rm polylog}}
\newcommand{\poly}{{\rm poly}}
% \newcommand{\vol}{\mathrm{vol}}
\newcommand{\supp}{\mathrm{supp}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\reg}{\text{reg}}

% epsilon wars
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}

% distributions
\newcommand{\Laplace}{\mathrm{Lap}}
\newcommand{\Lap}{\Laplace}
\newcommand{\Bin}{\mathrm{Bin}}


% remove text
\newcommand{\remove}[1]{}

%
% draftbox
%
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
        \begin{Large}%
          \textsc{Working Draft}%
        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}

% compact itemize and enumerate
\renewcommand{\labelitemi}{--}
\newenvironment{itm}
{\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]}
{\end{itemize}}
\newenvironment{enum}
{\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]}
{\end{enumerate}}

% control white space of list and display environments
%
%\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
%\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}
\def\mydatewithyear{\leavevmode\hbox{\the\year/\twodigits\month/\twodigits\day}}
\def\twodigits#1{\ifnum#1<10 0\fi\the#1}
\def\mydate{\leavevmode\hbox{\twodigits\month/\twodigits\day}}
\def\twodigits#1{\ifnum#1<10 0\fi\the#1}

% Macros for repeated theorems.
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newreptheorem{theorem}{Theorem}
\newreptheorem{corollary}{Corollary}
\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}




\newcounter{protocol}
\makeatletter
\newenvironment{protocol}[1][htb]{%
  \let\c@algorithm\c@protocol
  \renewcommand{\ALG@name}{Procedure}% Update algorithm name
  \begin{algorithm}[#1]%
  }{\end{algorithm}
}
\makeatother

